Analysing Fairness of Privacy-Utility Mobility Models

Preserving the individuals' privacy in sharing spatial-temporal datasets is critical to prevent re-identification attacks based on unique trajectories. Existing privacy techniques tend to propose ideal privacy-utility tradeoffs, however, largely ignore the fairness implications of mobility models and whether such techniques perform equally for different groups of users. The quantification between fairness and privacy-aware models is still unclear and there barely exists any defined sets of metrics for measuring fairness in the spatial-temporal context. In this work, we define a set of fairness metrics designed explicitly for human mobility, based on structural similarity and entropy of the trajectories. Under these definitions, we examine the fairness of two state-of-the-art privacy-preserving models that rely on GAN and representation learning to reduce the re-identification rate of users for data sharing. Our results show that while both models guarantee group fairness in terms of demographic parity, they violate individual fairness criteria, indicating that users with highly similar trajectories receive disparate privacy gain. We conclude that the tension between the re-identification task and individual fairness needs to be considered for future spatial-temporal data analysis and modelling to achieve a privacy-preserving fairness-aware setting.

==> cluster.tex <==
\begin{table*}[t]\small
   \centering
   \begin{tabular}{ccccccccc}
    \hline
    & \multirow{2}{*}{\shortstack{Metrics}} & \multirow{2}{*}{\shortstack{\#}} & \multicolumn{2}{|c|}{Original, P\% of (DIFF>0.2)} & \multicolumn{2}{c|}{Mo-PAE, P\% of (DIFF>0.2)} & \multicolumn{2}{c}{TrajGAN, P\% of (DIFF>0.2)} \\
    \cline{4-9}
       &  &  & \multicolumn{1}{|c}{Uniqueness} & \multicolumn{1}{c|}{Predictability}  & Privacy Gain  & \multicolumn{1}{c|}{Utility Decline}  & Privacy Gain & \multicolumn{1}{c}{Utility Decline}\\
       \cline{1-9}
       \multirow{8}{*}{\shortstack{MDC}} 
       & SE & 3419 & 10.50\% & 11.11\% & 87.69\% & 39.75\% & 41.65\% & 27.32\% \\
       & LE & 1215 & 8.31\% & 7.90\% & 88.81\% & 36.95\% & 41.32\% & 25.10\% \\
       & HE & 1334 & 12.89\% & 9.60\% & 86.88\% & 41.30\% & 38.23\% & 27.14\% \\       
       \hdashline
       & AE & 3124 & 12.64\% & 10.28\% & 87.10\% & 35.95\% & \textbf{45.26\%} & \textbf{29.42\%} \\
       \cline{2-9}
        & SSIM & 6150 & \textbf{14.57\%} & \textbf{13.17\%} & \textbf{88.98\%} & \textbf{42.02\%} & 39.50\% & 27.50\% \\
       \cline{2-9}
       & 4 Entropy & 164 & 6.10\% & 1.22\% & 84.76\% & \textbf{30.49\%} & 44.51\% & 27.44\% \\
       & 4 Entropy+SSIM & 155 & 6.45\% & 1.29\% & 83.87\% & 31.61\% & 43.23\% & 28.39\% \\
       %& AE/records & 501 & 8.18\% & 8.38\% & 86.83\% & 35.73\% & 42.91\% & 28.14\% \\
       %& All & 27 & \textbf{3.70\%} & \textbf{0.00\%} & \textbf{77.78\%} & 33.33\% & \textbf{37.04\%} & \textbf{18.52\%}\\
       \cline{1-9}
       \multirow{8}{*}{\shortstack{Geolife}} 
       & SE & 3462 & 57.91\% & 61.09\% & 94.14\% & 71.84\% & 67.85\% & 58.58\% \\
       & LE & 951 & 57.41\% & 61.20\% & 94.32\% & 71.50\% & 65.09\% & 56.05\% \\
       & HE & 761 & 61.37\% & \textbf{63.47\%} & 94.09\% & 70.43\% & 69.78\% & 58.87\% \\
       & AE & 2822 &  57.44\% & 59.36\% & 93.23\% & 72.96\% & 71.96\% & 58.54\% \\
       \cline{2-9}
       & SSIM & 6632 & 59.88\% & 61.49\% & 94.13\% & \textbf{74.77\%} & 63.53\% & \textbf{53.05\%} \\
       \cline{2-9}
       & 4 Entropy & 65 & 61.54\% & 58.46\% & 89.23\% & 66.15\% & \textbf{78.46\%} & \textbf{72.31\%} \\
       & 4 Entropy+SSIM & 64 & \textbf{62.50\%} & 57.81\% & 89.06\% & 65.63\% & 78.13\% & 71.88\% \\
       %& AE/records & 459 & 61.66\% & 58.82\% & \textbf{88.67\%} & 68.63\% & 76.03\% & 64.27\% \\
       %& All & 9 & \textbf{55.56\%} & \textbf{55.56\%} & \textbf{100.00\%} & \textbf{44.44\%} & \textbf{55.56\%} & 66.67\% \\
        \hline
    \end{tabular}
    
    \caption{Individual fairness based on SSIM and different types of entropies among different models and datasets.
    SE represents \textit{shannon entropy}; HE represents \textit{heatmap entropy}; LE represents \textit{lonlat entropy}; AE represents \textit{actual entropy}; \textit{4 Entropy} means the final chosen similar trajectories are restricted by SE, HE, LE and AE in the same time; same as the \textit{4 Entropy+SSIM}; AE/records is take the number of trajectories of each user into considerations; \textit{ALL} means the chosen similar trajectories are restricted by all of the above metrics. }
    \label{tab:IF}
\end{table*}

==> fml.tex <==

\subsection{Stages of Applying Fairness in Machine Learning}

 Fairness in ML can be achieved in three different stages: pre-processing the data, in-processing where the model is modified to become fair, and post-processing where the outcome of the model is tuned to meet the fairness criteria. 
 
{\em pre-processing:} Pre-processing methods concentrate on  removing representation bias and/or labelling bias in the training data in order to ensure fair balanced training data. For example, applicants of a certain gender might be up-weighted or down-weighted to retrain models and reduce disparities across different gender groups.
\\

 {\em in-processing:} %
In-processing approaches rely on adjusting the model during training to impose
fairness constraints or include fairness terms in the loss function to be
optimized. One in-processing strategy is representation learning via autoencoder
networks that are encouraged to learn features that are orthogonal to the
sensitive attribute--that is, they impose regularizing priors and/or penalty
terms to learn a latent representation $z$, which is both maximally informative
about the target variable $y$ and minimally informative about the sensitive
variable $s$. The Variational Fair Autoencoder from~\cite{louizos2017variational} and the Flexibly Fair Variational Autoencoder
(FFVAE) from~\cite{creager_flexibly_2019} are two prominent
examples of this approach. Adversarial debiasing, introduced in
\cite{zhang_mitigating_2018}, adds a discriminator sub-model to predict the
sensitive class label from $z$ and adds the negative discriminator loss to the
overall model loss function, encouraging the model to learn embeddings that are
minimally predictive of the sensitive variable.

\\

{\em post-processing:} Finally as most of the time in-processing approaches are not possible due to a lack of access to modifying the underlying model. The majority of the traditional linear algorithmic machine learning literature leverages   the post-processing approach. These class of fairness algorithms take an existing classifier and by treating it as a black box they aim to adjust the outcome. Such approaches also require access to the sensitive feature as input, so that they derive a transformation of the classifier's prediction to enforce the specified fairness constraints. The biggest advantage of threshold optimization is its simplicity and flexibility as it does not need to retrain the model. 
